Properties of the 15 February 2011 Flare Seismic Sources

The first near-side X-class flare of the Solar Cycle 24 occurred in February 2011 and produced a very strong seismic response in the photosphere. One sunquake was reported by Kosovichev (2011) followed by the discovery of a second sunquake by Zharkov et al (2011). The flare had a two-ribbon structure and was associated with a flux rope eruption and a halo coronal mass ejection (CME) as reported in the CACTus catalogue. Following the discovery of the second sunquake and the spatial association of both sources with the locations of the feet of the erupting flux rope (Zharkov et al 2011) we present here a more detailed analysis of the observed photospheric changes in and around the seismic sources. These sunquakes are quite unusual, taking place early in the impulsive stage of the flare, with the seismic sources showing little hard X-ray (HXR) emission, and strongest X-ray emission sources located in the flare ribbons. We present a directional time--distance diagram computed for the second source, which clearly shows a ridge corresponding to the travelling acoustic wave packet and find that the quake at the second source happened about 45 seconds to one minute earlier than the first source. Using acoustic holography we report different frequency responses of the two sources. We find strong downflows at both seismic locations and a supersonic horizontal motion at the second site of acoustic wave excitation.

==> solphys_rhodes_revision_2refs_1.tex <==
\begin{thebibliography}{43}
% BibTex style file: spr-mp-sola-cnd.bst (nameyear,cnd), 2011-09-16
\ifx \bisbn   \undefined \def \bisbn  #1{ISBN #1}\fi
\ifx \binits  \undefined \def \binits#1{#1}\fi
\ifx \bauthor  \undefined \def \bauthor#1{#1}\fi
\ifx \batitle  \undefined \def \batitle#1{#1}\fi
\ifx \bjtitle  \undefined \def \bjtitle#1{\textit{#1}}\fi
\ifx \bvolume  \undefined \def \bvolume#1{\textbf{#1}}\fi
\ifx \byear  \undefined \def \byear#1{#1}\fi
\ifx \bissue  \undefined \def \bissue#1{#1}\fi
\ifx \bfpage  \undefined \def \bfpage#1{#1}\fi
\ifx \blpage  \undefined \def \blpage #1{#1}\fi
\ifx \burl  \undefined \def \burl#1{\textsf{#1}}\fi
\ifx \href  \undefined \def \href#1#2{\textsf{#2}}\fi
\ifx \doiurl  \undefined \def
\doiurl#1{\href{http://dx.doi.org/#1}{\textsf{#1}}}\fi
\ifx \betal  \undefined \def \betal{\textit{et al.}}\fi
\ifx \binstitute  \undefined \def \binstitute#1{#1}\fi
\ifx \bctitle  \undefined \def \bctitle#1{#1}\fi
\ifx \beditor  \undefined \def \beditor#1{#1}\fi
\ifx \bpublisher  \undefined \def \bpublisher#1{#1}\fi
\ifx \bbtitle  \undefined \def \bbtitle#1{\textit{#1}}\fi
\ifx \bedition  \undefined \def \bedition#1{#1}\fi
\ifx \bseriesno  \undefined \def \bseriesno#1{\textbf{#1}}\fi
\ifx \blocation  \undefined \def \blocation#1{#1}\fi
\ifx \bsertitle  \undefined \def \bsertitle#1{\textit{#1}}\fi
\ifx \bsnm \undefined \def \bsnm#1{#1}\fi
\ifx \bsuffix \undefined \def \bsuffix#1{#1}\fi
\ifx \bparticle \undefined \def \bparticle#1{#1}\fi
\ifx \barticle \undefined \def \barticle#1{}\fi
\ifx \botherref \undefined \def \botherref#1{}\fi
\ifx \url \undefined \def \url#1{\textsf{#1}}\fi
\ifx \bchapter \undefined \def \bchapter#1{}\fi
\ifx \bbook \undefined \def \bbook#1{}\fi
\ifx \bcomment \undefined \def \bcomment#1{#1}\fi
\ifx \oauthor \undefined \def \oauthor#1{#1}\fi
\ifx \citeauthoryear \undefined \def \citeauthoryear#1{#1}\fi
\def \endbibitem {}
\ifx \bconflocation  \undefined \def \bconflocation#1{#1} \fi



\bibitem[\protect\citeauthoryear{{Alvarado-G{\'o}mez}, {Buitrago-Casas}, {Mart{\'{\i}}nez-Oliveros}
  \textit{et~al.}}{2012}]{ABMLHC2012}
\begin{botherref}
\oauthor{\bsnm{{Alvarado-G{\'o}mez}}, \binits{J.D.}},
\oauthor{\bsnm{{Buitrago-Casas}}, \binits{J.C.}},
\oauthor{\bsnm{{Mart{\'{\i}}nez-Oliveros}}, \binits{J.C.}},
\oauthor{\bsnm{{Lindsey}}, \binits{C.}},
\oauthor{\bsnm{{Hudson}}, \binits{H.}},
\oauthor{\bsnm{{Calvo-Mozo}}, \binits{B.}}:
2012,
\textit{\solphys},
131.
ADS:\adsurl{2012SoPh..tmp..131A},
doi:\doiurl{10.1007/s11207-012-0009-6}.
\end{botherref}
\endbibitem

\bibitem[\protect\citeauthoryear{{Besliu-Ionescu}, {Donea}, {Cally}
  \textit{et~al.}}{2005}]{Besliu2005}
\begin{bchapter}
\bauthor{\bsnm{{Besliu-Ionescu}}, \binits{D.}},
\bauthor{\bsnm{{Donea}}, \binits{A.}},
\bauthor{\bsnm{{Cally}}, \binits{P.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{2005},
In: Danesy,~D., Poedts,~S.,De Groof,~A., Andries,J. (eds.), \bbtitle{The Dynamic Sun: Challenges for Theory and Observations},
\bseriesno{SP-600},
ESA, Noordwijk, 111.
\end{bchapter}
ADS:\adsurl{2005ESASP.600E.111B}.
\endbibitem

\bibitem[\protect\citeauthoryear{{Besliu-Ionescu}, {Donea}, {Cally}
  \textit{et~al.}}{2006}]{Besilu2006Mclass}
\begin{bchapter}
\bauthor{\bsnm{{Besliu-Ionescu}}, \binits{D.}},
\bauthor{\bsnm{{Donea}}, \binits{A.-C.}},
\bauthor{\bsnm{{Cally}}, \binits{P.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{2006},
In: Fletcher, K., Thompson, M.J. (eds.), \bbtitle{Proceedings of SOHO 18/GONG 2006/HELAS I, Beyond the spherical
  Sun},
\bseriesno{SP-624},
ESA, Noordwijk, 67.
\end{bchapter}
ADS:\adsurl{2006ESASP.624E..67B}.
\endbibitem

\bibitem[\protect\citeauthoryear{{Braun} and {Lindsey}}{1999}]{BL1999}
\begin{barticle}
\bauthor{\bsnm{{Braun}}, \binits{D.~C.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{1999},
\bjtitle{\apjl}
\bvolume{513},
\bfpage{L79}.
ADS:\adsurl{1999ApJÉ513L..79B},
doi:\doiurl{10.1086/311897}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Braun} and {Lindsey}}{2000}]{BL2000a}
\begin{barticle}
\bauthor{\bsnm{{Braun}}, \binits{D.C.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{2000},
\bjtitle{\solphys}
\bvolume{192},
\bfpage{285}.
ADS:\adsurl{2000SoPh..192..285B}, 
doi:\doiurl{10.1023/A:1005287419566}
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Cally}}{2000}]{C2000}
\begin{barticle}
\bauthor{\bsnm{{Cally}}, \binits{P.S.}}:
\byear{2000},
\bjtitle{\solphys}
\bvolume{192},
\bfpage{395}.
ADS:\adsurl{2000SoPh..192..395C}, 
doi:\doiurl{10.1023/A:1005213002513}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Christensen-Dalsgaard}, {Dappen}, {Ajukov}
  \textit{et~al.}}{1996}]{CDModel}
\begin{barticle}
\bauthor{\bsnm{{Christensen-Dalsgaard}}, \binits{J.}},
\bauthor{\bsnm{{Dappen}}, \binits{W.}},
\bauthor{\bsnm{{Ajukov}}, \binits{S.V.}},
\bauthor{\bsnm{{Anderson}}, \binits{E.R.}},
\bauthor{\bsnm{{Antia}}, \binits{H.M.}},
\bauthor{\bsnm{{Basu}}, \binits{S.}},
\bauthor{\bsnm{{Baturin}}, \binits{V.A.}},
\bauthor{\bsnm{{Berthomieu}}, \binits{G.}},
\bauthor{\bsnm{{Chaboyer}}, \binits{B.}},
\bauthor{\bsnm{{Chitre}}, \binits{S.M.}},
\bauthor{\bsnm{{Cox}}, \binits{A.N.}},
\bauthor{\bsnm{{Demarque}}, \binits{P.}},
\bauthor{\bsnm{{Donatowicz}}, \binits{J.}},
\bauthor{\bsnm{{Dziembowski}}, \binits{W.A.}},
\bauthor{\bsnm{{Gabriel}}, \binits{M.}},
\bauthor{\bsnm{{Gough}}, \binits{D.O.}},
\bauthor{\bsnm{{Guenther}}, \binits{D.B.}},
\bauthor{\bsnm{{Guzik}}, \binits{J.A.}},
\bauthor{\bsnm{{Harvey}}, \binits{J.W.}},
\bauthor{\bsnm{{Hill}}, \binits{F.}},
\bauthor{\bsnm{{Houdek}}, \binits{G.}},
\bauthor{\bsnm{{Iglesias}}, \binits{C.A.}},
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}},
\bauthor{\bsnm{{Leibacher}}, \binits{J.W.}},
\bauthor{\bsnm{{Morel}}, \binits{P.}},
\bauthor{\bsnm{{Proffitt}}, \binits{C.R.}},
\bauthor{\bsnm{{Provost}}, \binits{J.}},
\bauthor{\bsnm{{Reiter}}, \binits{J.}},
\bauthor{\bsnm{{Rhodes}}, \binits{E.J.} \bsuffix{Jr.}},
\bauthor{\bsnm{{Rogers}}, \binits{F.J.}},
\bauthor{\bsnm{{Roxburgh}}, \binits{I.W.}},
\bauthor{\bsnm{{Thompson}}, \binits{M.J.}},
\bauthor{\bsnm{{Ulrich}}, \binits{R.K.}}:
\byear{1996},
\bjtitle{Science}
\bvolume{272},
\bfpage{1286}.
doi:\doiurl{10.1126/science.272.5266.1286}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Donea}}{2011}]{donea11}
\begin{barticle}
\bauthor{\bsnm{{Donea}}, \binits{A.}}:
\byear{2011},
\bjtitle{\ssr}
\bvolume{158},
\bfpage{451}.
doi:\doiurl{10.1007/s11214-011-9787-7}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Donea} and {Lindsey}}{2005}]{DL2005}
\begin{barticle}
\bauthor{\bsnm{{Donea}}, \binits{A.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{2005},
\bjtitle{\apj}
\bvolume{630},
\bfpage{1168}.
doi:\doiurl{10.1086/432155}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Donea}, {Braun}, and
  {Lindsey}}{1999}]{Donea1999}
\begin{barticle}
\bauthor{\bsnm{{Donea}}, \binits{A.}},
\bauthor{\bsnm{{Braun}}, \binits{D.C.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}}:
\byear{1999},
\bjtitle{\apjl}
\bvolume{513},
\bfpage{L143}.
doi:\doiurl{10.1086/311915}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{Donea, Lindsey, and Braun}{2000}]{donea2000}
\begin{barticle}
\bauthor{\bsnm{Donea}, \binits{A.-C.}},
\bauthor{\bsnm{Lindsey}, \binits{C.}},
\bauthor{\bsnm{Braun}, \binits{D.C.}}:
\byear{2000},
\bjtitle{\solphys}
\bvolume{192}(\bissue{1}),
\bfpage{321}.
ADS:\adsurl{2000SoPh..192..321D}, 
doi:\doiurl{10.1023/A:1005280327665}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Donea}, {Besliu-Ionescu}, {Cally}
 \textit{et~al.}}{2006}]{Donea2006list}
\begin{barticle}
\bauthor{\bsnm{Donea}, \binits{A.C.}},
\bauthor{\bsnm{Besliu-Ionescu}, \binits{D.}},
\bauthor{\bsnm{Cally}, \binits{P.}},
\bauthor{\bsnm{Lindsey}, \binits{C.}}:
\byear{2006},
In: Leibacher, J., Stein, R.F., Uitenbroek,  H. (eds),
\bjtitle{Solar MHD Theory and Observations: A High Spatial Resolution
  Perspective}
\bvolume{CS-354},
Astron. Soc. Pacific, San Francisco,
\bfpage{204}.
ADS:\adsurl{2006ASPC..354..204D}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Duvall}, {Jefferies}, {Harvey} 
\textit{et~al.}}{1993}]{Duvall1993}
\begin{barticle}
\bauthor{\bsnm{{Duvall}}, \binits{T.L.} \bsuffix{Jr.}},
\bauthor{\bsnm{{Jefferies}}, \binits{S.M.}},
\bauthor{\bsnm{{Harvey}}, \binits{J.W.}},
\bauthor{\bsnm{{Pomerantz}}, \binits{M.A.}}:
\byear{1993},
\bjtitle{\nat}
\bvolume{362},
\bfpage{430}.
doi:\doiurl{10.1038/362430a0}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Duvall}, {Kosovichev},  {Scherrer}
\textit{et~al.}}{1997}]{Duvall1997}
\begin{barticle}
\bauthor{\bsnm{{Duvall}}, \binits{T.L.} \bsuffix{Jr.}},
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}},
\bauthor{\bsnm{{Scherrer}}, \binits{P.H.}},
\bauthor{\bsnm{{Bogart}}, \binits{R.S.}},
\bauthor{\bsnm{{Bush}}, \binits{R.I.}},
\bauthor{\bsnm{{de Forest}}, \binits{C.}},
\bauthor{\bsnm{{Hoeksema}}, \binits{J.T.}},
\bauthor{\bsnm{{Schou}}, \binits{J.}},
\bauthor{\bsnm{{Saba}}, \binits{J.L.R.}},
\bauthor{\bsnm{{Tarbell}}, \binits{T.D.}},
\bauthor{\bsnm{{Title}}, \binits{A.M.}},
\bauthor{\bsnm{{Wolfson}}, \binits{C.J.}},
\bauthor{\bsnm{{Milford}}, \binits{P.N.}}:
\byear{1997},
\bjtitle{\solphys}
\bvolume{170},
\bfpage{63}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Felipe}, {Khomenko}, and
  {Collados}}{2010}]{Felipe2010}
\begin{barticle}
\bauthor{\bsnm{{Felipe}}, \binits{T.}},
\bauthor{\bsnm{{Khomenko}}, \binits{E.}},
\bauthor{\bsnm{{Collados}}, \binits{M.}}:
\byear{2010},
\bjtitle{\apj}
\bvolume{719},
\bfpage{357}.
doi:\doiurl{10.1088/0004-637X/719/1/357}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Fisher}, {Welsch}, and
  {Abbett}}{2012}]{Fisher2011}
\begin{botherref}
\oauthor{\bsnm{{Fisher}}, \binits{G.H.}},
\oauthor{\bsnm{{Welsch}}, \binits{B.T.}},
\oauthor{\bsnm{{Abbett}}, \binits{W.P.}}:
2012,
\textit{\solphys},
325.
ADS:\adsurl{2012SoPh..277..153F},
doi:\doiurl{10.1007/s11207-011-9816-4}.
\end{botherref}
\endbibitem

\bibitem[\protect\citeauthoryear{{Fisher}, {Bercik}, {Welsch} 
\textit{et~al.}}{2012}]{Fisher2012}
\begin{barticle}
\bauthor{\bsnm{Fisher}, \binits{G.}},
\bauthor{\bsnm{Bercik}, \binits{D.}},
\bauthor{\bsnm{Welsch}, \binits{B.}},
\bauthor{\bsnm{Hudson}, \binits{H.}}:
\byear{2012},
\bjtitle{Solar Physics}
\bvolume{277},
\bfpage{59}.
ADS:\adsurl{2012SoPh..277...59F}, 
doi:\doiurl{10.1007/s11207-011-9907-2}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Hudson}, {Fisher}, and
  {Welsch}}{2008}]{Hudson08}
\begin{bchapter}
\bauthor{\bsnm{{Hudson}}, \binits{H.S.}},
\bauthor{\bsnm{{Fisher}}, \binits{G.H.}},
\bauthor{\bsnm{{Welsch}}, \binits{B.T.}}:
\byear{2008},
In: \beditor{\bsnm{{Howe,~R., Komm,~R.~W., Balasubramaniam,~K.~S., Petrie,~G.~J.~D.}}} (eds.)
\bbtitle{Subsurface and Atmospheric Influences on Solar Activity}
\bseriesno{CS-383},
Astron. Soc. Pacific, San Francisco,
\bfpage{221}.
ADS:\adsurl{2008ASPC..383..221H}.
\end{bchapter}
\endbibitem

\bibitem[\protect\citeauthoryear{{Kosovichev}}{2006}]{K2006}
\begin{barticle}
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}}:
\byear{2006},
\bjtitle{\solphys}
\bvolume{238},
\bfpage{1}.
ADS:\adsurl{2006SoPh..238....1K},
doi:\doiurl{10.1007/s11207-006-0190-6}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Kosovichev}}{2007}]{Kosovichev2007}
\begin{barticle}
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}}:
\byear{2007},
\bjtitle{\apjl}
\bvolume{670},
\bfpage{L65}.
doi:\doiurl{10.1086/524036}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Kosovichev}}{2011}]{Kosovichev2011}
\begin{barticle}
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}}:
\byear{2011},
\bjtitle{\apjl}
\bvolume{734},
\bfpage{L15}.
doi:\doiurl{10.1088/2041-8205/734/1/L15}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Kosovichev} and {Zharkova}}{1998}]{kz1998}
\begin{barticle}
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}},
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}}:
\byear{1998},
\bjtitle{\nat}
\bvolume{393},
\bfpage{317}.
doi:\doiurl{10.1038/30629}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Kosovichev}, {Duvall}, and
  {Scherrer}}{2000}]{Kosovichev2000}
\begin{barticle}
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}},
\bauthor{\bsnm{{Duvall}}, \binits{T.L..} \bsuffix{Jr.}},
\bauthor{\bsnm{{Scherrer}}, \binits{P.H.}}:
\byear{2000},
\bjtitle{\solphys}
\bvolume{192},
\bfpage{159}.
ADS:\adsurl{2000SoPh..192..159K},
doi:\doiurl{10.1023/A:1005251208431}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Lin}, {Dennis}, {Hurford} 
\textit{et~al.}}{2002}]{lin02}
\begin{barticle}
\bauthor{\bsnm{{Lin}}, \binits{R.P.}},
\bauthor{\bsnm{{Dennis}}, \binits{B.R.}},
\bauthor{\bsnm{{Hurford}}, \binits{G.J.}},
\bauthor{\bsnm{{Smith}}, \binits{D.M.}},
\bauthor{\bsnm{{Zehnder}}, \binits{A.}},
\bauthor{\bsnm{{Harvey}}, \binits{P.R.}},
\bauthor{\bsnm{{Curtis}}, \binits{D.W.}},
\bauthor{\bsnm{{Pankow}}, \binits{D.}},
\bauthor{\bsnm{{Turin}}, \binits{P.}},
\bauthor{\bsnm{{Bester}}, \binits{M.}},
\bauthor{\bsnm{{Csillaghy}}, \binits{A.}},
\bauthor{\bsnm{{Lewis}}, \binits{M.}},
\bauthor{\bsnm{{Madden}}, \binits{N.}},
\bauthor{\bsnm{{van Beek}}, \binits{H.F.}},
\bauthor{\bsnm{{Appleby}}, \binits{M.}},
\bauthor{\bsnm{{Raudorf}}, \binits{T.}},
\bauthor{\bsnm{{McTiernan}}, \binits{J.}},
\bauthor{\bsnm{{Ramaty}}, \binits{R.}},
\bauthor{\bsnm{{Schmahl}}, \binits{E.}},
\bauthor{\bsnm{{Schwartz}}, \binits{R.}},
\bauthor{\bsnm{{Krucker}}, \binits{S.}},
\bauthor{\bsnm{{Abiad}}, \binits{R.}},
\bauthor{\bsnm{{Quinn}}, \binits{T.}},
\bauthor{\bsnm{{Berg}}, \binits{P.}},
\bauthor{\bsnm{{Hashii}}, \binits{M.}},
\bauthor{\bsnm{{Sterling}}, \binits{R.}},
\bauthor{\bsnm{{Jackson}}, \binits{R.}},
\bauthor{\bsnm{{Pratt}}, \binits{R.}},
\bauthor{\bsnm{{Campbell}}, \binits{R.D.}},
\bauthor{\bsnm{{Malone}}, \binits{D.}},
\bauthor{\bsnm{{Landis}}, \binits{D.}},
\bauthor{\bsnm{{Barrington-Leigh}}, \binits{C.P.}},
\bauthor{\bsnm{{Slassi-Sennou}}, \binits{S.}},
\bauthor{\bsnm{{Cork}}, \binits{C.}},
\bauthor{\bsnm{{Clark}}, \binits{D.}},
\bauthor{\bsnm{{Amato}}, \binits{D.}},
\bauthor{\bsnm{{Orwig}}, \binits{L.}},
\bauthor{\bsnm{{Boyle}}, \binits{R.}},
\bauthor{\bsnm{{Banks}}, \binits{I.S.}},
\bauthor{\bsnm{{Shirey}}, \binits{K.}},
\bauthor{\bsnm{{Tolbert}}, \binits{A.K.}},
\bauthor{\bsnm{{Zarro}}, \binits{D.}},
\bauthor{\bsnm{{Snow}}, \binits{F.}},
\bauthor{\bsnm{{Thomsen}}, \binits{K.}},
\bauthor{\bsnm{{Henneck}}, \binits{R.}},
\bauthor{\bsnm{{McHedlishvili}}, \binits{A.}},
\bauthor{\bsnm{{Ming}}, \binits{P.}},
\bauthor{\bsnm{{Fivian}}, \binits{M.}},
\bauthor{\bsnm{{Jordan}}, \binits{J.}},
\bauthor{\bsnm{{Wanner}}, \binits{R.}},
\bauthor{\bsnm{{Crubb}}, \binits{J.}},
\bauthor{\bsnm{{Preble}}, \binits{J.}},
\bauthor{\bsnm{{Matranga}}, \binits{M.}},
\bauthor{\bsnm{{Benz}}, \binits{A.}},
\bauthor{\bsnm{{Hudson}}, \binits{H.}},
\bauthor{\bsnm{{Canfield}}, \binits{R.C.}},
\bauthor{\bsnm{{Holman}}, \binits{G.D.}},
\bauthor{\bsnm{{Crannell}}, \binits{C.}},
\bauthor{\bsnm{{Kosugi}}, \binits{T.}},
\bauthor{\bsnm{{Emslie}}, \binits{A.G.}},
\bauthor{\bsnm{{Vilmer}}, \binits{N.}},
\bauthor{\bsnm{{Brown}}, \binits{J.C.}},
\bauthor{\bsnm{{Johns-Krull}}, \binits{C.}},
\bauthor{\bsnm{{Aschwanden}}, \binits{M.}},
\bauthor{\bsnm{{Metcalf}}, \binits{T.}},
\bauthor{\bsnm{{Conway}}, \binits{A.}}:
\byear{2002},
\bjtitle{\solphys}
\bvolume{210},
\bfpage{3}.
doi:\doiurl{10.1023/A:1022428818870}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Lindsey} and {Braun}}{2000}]{LB2000}
\begin{barticle}
\bauthor{\bsnm{{Lindsey}}, \binits{C.}},
\bauthor{\bsnm{{Braun}}, \binits{D.C.}}:
\byear{2000},
\bjtitle{\solphys}
\bvolume{192},
\bfpage{261}.
ADS:\adsurl{2000SoPh..192..261L},
doi:\doiurl{10.1023/A:1005227200911}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{Lindsey and Braun}{2004}]{LB2004}
\begin{barticle}
\bauthor{\bsnm{Lindsey}, \binits{C.}},
\bauthor{\bsnm{Braun}, \binits{D.C.}}:
\byear{2004},
\bjtitle{Astrophys. J. Supp. Ser.}
\bvolume{155},
\bfpage{209}.
ADS:\adsurl{2004ApJS..155..209},
doi:\doiurl{10.1086/424736}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Mart{\'{\i}}nez-Oliveros}, {Moradi}, and
  {Donea}}{2008}]{Martinez2008a}
\begin{barticle}
\bauthor{\bsnm{{Mart{\'{\i}}nez-Oliveros}}, \binits{J.C.}},
\bauthor{\bsnm{{Moradi}}, \binits{H.}},
\bauthor{\bsnm{{Donea}}, \binits{A.}}:
\byear{2008},
\bjtitle{\solphys}
\bvolume{251},
\bfpage{613}.
ADS:\adsurl{2008SoPh..251..613M},
doi:\doiurl{10.1007/s11207-008-9122-y}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Matthews}, {Zharkov}, and
  {Zharkova}}{2011}]{MZZ2011}
\begin{barticle}
\bauthor{\bsnm{{Matthews}}, \binits{S.A.}},
\bauthor{\bsnm{{Zharkov}}, \binits{S.}},
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}}:
\byear{2011},
\bjtitle{\apj}
\bvolume{739},
\bfpage{71}.
doi:\doiurl{10.1088/0004-637X/739/2/71}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Moradi}, {Donea}, {Lindsey} 
\textit{et~al.}}{2007}]{Moradi2007}
\begin{barticle}
\bauthor{\bsnm{{Moradi}}, \binits{H.}},
\bauthor{\bsnm{{Donea}}, \binits{A.}},
\bauthor{\bsnm{{Lindsey}}, \binits{C.}},
\bauthor{\bsnm{{Besliu-Ionescu}}, \binits{D.}},
\bauthor{\bsnm{{Cally}}, \binits{P.S.}}:
\byear{2007},
\bjtitle{\mnras}
\bvolume{374},
\bfpage{1155}.
doi:\doiurl{10.1111/j.1365-2966.2006.11234.x}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Moradi}, {Baldner}, {Birch} 
\textit{et~al.}}{2010}]{Moradi2010}
\begin{barticle}
\bauthor{\bsnm{{Moradi}}, \binits{H.}},
\bauthor{\bsnm{{Baldner}}, \binits{C.}},
\bauthor{\bsnm{{Birch}}, \binits{A.C.}},
\bauthor{\bsnm{{Braun}}, \binits{D.C.}},
\bauthor{\bsnm{{Cameron}}, \binits{R.H.}},
\bauthor{\bsnm{{Duvall}}, \binits{T.L.}},
\bauthor{\bsnm{{Gizon}}, \binits{L.}},
\bauthor{\bsnm{{Haber}}, \binits{D.}},
\bauthor{\bsnm{{Hanasoge}}, \binits{S.M.}},
\bauthor{\bsnm{{Hindman}}, \binits{B.W.}},
\bauthor{\bsnm{{Jackiewicz}}, \binits{J.}},
\bauthor{\bsnm{{Khomenko}}, \binits{E.}},
\bauthor{\bsnm{{Komm}}, \binits{R.}},
\bauthor{\bsnm{{Rajaguru}}, \binits{P.}},
\bauthor{\bsnm{{Rempel}}, \binits{M.}},
\bauthor{\bsnm{{Roth}}, \binits{M.}},
\bauthor{\bsnm{{Schlichenmaier}}, \binits{R.}},
\bauthor{\bsnm{{Schunker}}, \binits{H.}},
\bauthor{\bsnm{{Spruit}}, \binits{H.C.}},
\bauthor{\bsnm{{Strassmeier}}, \binits{K.G.}},
\bauthor{\bsnm{{Thompson}}, \binits{M.J.}},
\bauthor{\bsnm{{Zharkov}}, \binits{S.}}:
\byear{2010},
\bjtitle{\solphys}
\bvolume{267},
\bfpage{1}.
ADS:\adsurl{2010SoPh..267....1M},
doi:\doiurl{10.1007/s11207-010-9630-4}.
\end{barticle}
\endbibitem


\bibitem[\protect\citeauthoryear{{Scherrer}, {Schou}, {Bush}
  \textit{et~al.}}{2012}]{ScherrerHMI2011}
\begin{barticle}
\bauthor{\bsnm{{Scherrer}}, \binits{P.H.}},
\bauthor{\bsnm{{Schou}}, \binits{J.}},
\bauthor{\bsnm{{Bush}}, \binits{R.I.}},
\bauthor{\bsnm{{Kosovichev}}, \binits{A.G.}},
\bauthor{\bsnm{{Bogart}}, \binits{R.S.}},
\bauthor{\bsnm{{Hoeksema}}, \binits{J.T.}},
\bauthor{\bsnm{{Liu}}, \binits{Y.}},
\bauthor{\bsnm{{Duvall}}, \binits{T.L.}},
\bauthor{\bsnm{{Zhao}}, \binits{J.}},
\bauthor{\bsnm{{Title}}, \binits{A.M.}},
\bauthor{\bsnm{{Schrijver}}, \binits{C.J.}},
\bauthor{\bsnm{{Tarbell}}, \binits{T.D.}},
\bauthor{\bsnm{{Tomczyk}}, \binits{S.}}:
\byear{2012},
\bjtitle{\solphys}
\bvolume{275},
\bfpage{207}.
ADS:\adsurl{2012SoPh..275..207S},
doi:\doiurl{10.1007/s11207-011-9834-2}.
\end{barticle}
\endbibitem



\bibitem[\protect\citeauthoryear{{Schou}, {Scherrer}, {Bush} 
\textit{et~al.}}{2012}]{Schou2011hmi}
\begin{barticle}
\bauthor{\bsnm{{Schou}}, \binits{J.}},
\bauthor{\bsnm{{Scherrer}}, \binits{P.H.}},
\bauthor{\bsnm{{Bush}}, \binits{R.I.}},
\bauthor{\bsnm{{Wachter}}, \binits{R.}},
\bauthor{\bsnm{{Couvidat}}, \binits{S.}},
\bauthor{\bsnm{{Rabello-Soares}}, \binits{M.C.}},
\bauthor{\bsnm{{Bogart}}, \binits{R.S.}},
\bauthor{\bsnm{{Hoeksema}}, \binits{J.T.}},
\bauthor{\bsnm{{Liu}}, \binits{Y.}},
\bauthor{\bsnm{{Duvall}}, \binits{T.L.}},
\bauthor{\bsnm{{Akin}}, \binits{D.J.}},
\bauthor{\bsnm{{Allard}}, \binits{B.A.}},
\bauthor{\bsnm{{Miles}}, \binits{J.W.}},
\bauthor{\bsnm{{Rairden}}, \binits{R.}},
\bauthor{\bsnm{{Shine}}, \binits{R.A.}},
\bauthor{\bsnm{{Tarbell}}, \binits{T.D.}},
\bauthor{\bsnm{{Title}}, \binits{A.M.}},
\bauthor{\bsnm{{Wolfson}}, \binits{C.J.}},
\bauthor{\bsnm{{Elmore}}, \binits{D.F.}},
\bauthor{\bsnm{{Norton}}, \binits{A.A.}},
\bauthor{\bsnm{{Tomczyk}}, \binits{S.}}:
\byear{2012},
\bjtitle{\solphys}
\bvolume{275},
\bfpage{229}.
ADS:\adsurl{2012SoPh..275..229S},
doi:\doiurl{10.1007/s11207-011-9842-2}.
\end{barticle}
\endbibitem


\bibitem[\protect\citeauthoryear{{Schrijver}, {Aulanier}, {Title}
  \textit{et~al.}}{2011}]{Schrijver2011}
\begin{barticle}
\bauthor{\bsnm{{Schrijver}}, \binits{C.J.}},
\bauthor{\bsnm{{Aulanier}}, \binits{G.}},
\bauthor{\bsnm{{Title}}, \binits{A.M.}},
\bauthor{\bsnm{{Pariat}}, \binits{E.}},
\bauthor{\bsnm{{Delann{\'e}e}}, \binits{C.}}:
\byear{2011},
\bjtitle{\apj}
\bvolume{738},
\bfpage{167}.
doi:\doiurl{10.1088/0004-637X/738/2/167}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Schunker} and {Cally}}{2006}]{Schunker2006}
\begin{barticle}
\bauthor{\bsnm{{Schunker}}, \binits{H.}},
\bauthor{\bsnm{{Cally}}, \binits{P.S.}}:
\byear{2006},
\bjtitle{\mnras}
\bvolume{372},
\bfpage{551}.
doi:\doiurl{10.1111/j.1365-2966.2006.10855.x}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Shelyag}, {Zharkov}, {Fedun} 
\textit{et~al.}}{2009}]{SZ09}
\begin{barticle}
\bauthor{\bsnm{{Shelyag}}, \binits{S.}},
\bauthor{\bsnm{{Zharkov}}, \binits{S.}},
\bauthor{\bsnm{{Fedun}}, \binits{V.}},
\bauthor{\bsnm{{Erd{\'e}lyi}}, \binits{R.}},
\bauthor{\bsnm{{Thompson}}, \binits{M.J.}}:
\byear{2009},
\bjtitle{\aap}
\bvolume{501},
\bfpage{735}.
doi:\doiurl{10.1051/0004-6361/200911709}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Sudol} and {Harvey}}{2005}]{Sudol2005}
\begin{barticle}
\bauthor{\bsnm{{Sudol}}, \binits{J.J.}},
\bauthor{\bsnm{{Harvey}}, \binits{J.W.}}:
\byear{2005},
\bjtitle{\apj}
\bvolume{635},
\bfpage{647}.
doi:\doiurl{10.1086/497361}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Sun}, {Hoeksema}, {Liu} 
\textit{et~al.}}{2012}]{XSun2012}
\begin{barticle}
\bauthor{\bsnm{{Sun}}, \binits{X.}},
\bauthor{\bsnm{{Hoeksema}}, \binits{J.T.}},
\bauthor{\bsnm{{Liu}}, \binits{Y.}},
\bauthor{\bsnm{{Wiegelmann}}, \binits{T.}},
\bauthor{\bsnm{{Hayashi}}, \binits{K.}},
\bauthor{\bsnm{{Chen}}, \binits{Q.}},
\bauthor{\bsnm{{Thalmann}}, \binits{J.}}:
\byear{2012},
\bjtitle{\apj}
\bvolume{748},
\bfpage{77}.
doi:\doiurl{10.1088/0004-637X/748/2/77}.
\end{barticle}
\endbibitem


\bibitem[\protect\citeauthoryear{{Wolff}}{1972}]{wolff72}
\begin{barticle}
\bauthor{\bsnm{{Wolff}}, \binits{C.L.}}:
\byear{1972},
\bjtitle{\apj}
\bvolume{176},
\bfpage{833}.
doi:\doiurl{10.1086/151680}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Zharkov}, {Nicholas}, and
  {Thompson}}{2007}]{ZNT2007}
\begin{barticle}
\bauthor{\bsnm{{Zharkov}}, \binits{S.}},
\bauthor{\bsnm{{Nicholas}}, \binits{C.J.}},
\bauthor{\bsnm{{Thompson}}, \binits{M.J.}}:
\byear{2007},
\bjtitle{Astron. Nachr.}
\bvolume{328},
\bfpage{240}.
doi:\doiurl{10.1002/asna.200610744}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Zharkov}, {Zharkova}, and
  {Matthews}}{2011}]{ZH2011}
\begin{barticle}
\bauthor{\bsnm{{Zharkov}}, \binits{S.}},
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}},
\bauthor{\bsnm{{Matthews}}, \binits{S.A.}}:
\byear{2011},
\bjtitle{\apj}
\bvolume{739},
\bfpage{70}.
doi:\doiurl{10.1088/0004-637X/739/2/70}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Zharkov}, {Green}, {Matthews} 
\textit{et~al.}}{2011}]{ZGMZ2011}
\begin{barticle}
\bauthor{\bsnm{{Zharkov}}, \binits{S.}},
\bauthor{\bsnm{{Green}}, \binits{L.M.}},
\bauthor{\bsnm{{Matthews}}, \binits{S.A.}},
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}}:
\byear{2011},
\bjtitle{\apjl}
\bvolume{741},
\bfpage{L35}.
doi:\doiurl{10.1088/2041-8205/741/2/L35}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Zharkova} and {Zharkov}}{2007}]{Zharkova07}
\begin{barticle}
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}},
\bauthor{\bsnm{{Zharkov}}, \binits{S.I.}}:
\byear{2007},
\bjtitle{\apj}
\bvolume{664},
\bfpage{573}.
doi:\doiurl{10.1086/518731}.
\end{barticle}
\endbibitem

\bibitem[\protect\citeauthoryear{{Zharkova}, {Zharkov}, {Ipson}
  \textit{et~al.}}{2005}]{Zharkova2005}
\begin{barticle}
\bauthor{\bsnm{{Zharkova}}, \binits{V.V.}},
\bauthor{\bsnm{{Zharkov}}, \binits{S.I.}},
\bauthor{\bsnm{{Ipson}}, \binits{S.S.}},
\bauthor{\bsnm{{Benkhalil}}, \binits{A.K.}}:
\byear{2005},
\bjtitle{J. Geophys. Res.}
\bvolume{110}(\bissue{A9}),
\bfpage{8104}.
doi:\doiurl{10.1029/2004JA010934}.
\end{barticle}
\endbibitem

\end{thebibliography}

